An integrated light management system with real-time light measurement and human perception

Illumination is important for well-being, productivity and safety across several environments, including offices, retail shops and industrial warehouses. Current techniques for setting up lighting require extensive and expert support and need to be repeated if the scene changes. Here we propose the first fully-automated light management system (LMS) which measures lighting in real-time, leveraging an RGBD sensor and a radiosity-based light propagation model. Thanks to the integration of light distribution and perception curves into the radiosity, we outperform a commercial software (Relux) on a newly introduced dataset. Furthermore, our proposed LMS is the first to estimate both the presence and the attention of the people in the environment, as well as their light perception. Our new LMS adapts therefore lighting to the scene and human activity and it is capable of saving up to 66%, as we experimentally quantify,without compromising the lighting quality.

==> sections/appendices.tex <==
\appendices
\section{Proof of the First Zonklar Equation}
Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.

==> sections/bibitem_bibliography.tex <==
\begin{thebibliography}{99}
\bibitem[Kopka and Daly(2003)]{R1}
Kopka~H and Daly~PW (2003) \textit{A Guide to \LaTeX}, 4th~edn.
Addison-Wesley.

\bibitem[Lamport(1994)]{R2}
Lamport~L (1994) \textit{\LaTeX: a Document Preparation System},
2nd~edn. Addison-Wesley.

\bibitem[Mittelbach and Goossens(2004)]{R3}
Mittelbach~F and Goossens~M (2004) \textit{The \LaTeX\ Companion},
2nd~edn. Addison-Wesley.

\end{thebibliography}

==> sections/bio.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:
\vspace{46pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pics/theodore.png}}]{Dr. Theodore Tsesmelis}
(t.tsemelis@osram.com - Parkring 33, 85748 Munich, Germany) is currently a computer vision researcher at the Computer Vision Department at OSRAM GmbH in Germany. Currently he is applying research and development regarding smart workspace management with the use of computer vision and machine learning. Other research interests involve reconstruction and recognition of 3D scenes, the scene material and object properties, and the estimation of lighting propagation.
\end{IEEEbiography}

\vspace{-23pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pics/irtiza.png}}]{Dr. Irtiza Hasan}
(irtiza.hasan@inceptioniai.org - Al Bustan office, tower Al Bustan, Abu Dhabi, UAE) is currently a research associate at Inception Institute of Artificial Intelligence (IIAI). His interests involve object detection, multi-object tracking, activity forecasting and pose estimation. 
\end{IEEEbiography}

\vspace{-28pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pics/marco.jpg}}]{Prof. Marco Cristani}
(marco.cristani@univr.it - Ca' Vignal 2, Strada le Grazie 15, 37134 Verona, Italy) is an Associate Professor (Professore Associato) at Computer Science Department, University of Verona. My main research interests are in statistical pattern recognition (mainly deep learning and generative modeling) and computer vision, with emphasis on social signal processing, \ie, how to model human activities with computer vision tools, following social psychology principia. In particular, I'm interested in fashion modeling (clothing parsing, recommendation, attribute learning) and how fashion is related to personality. Other interests are on video surveillance applications, such as human activity modeling, people re-identification and pedestrian detection.
\end{IEEEbiography}

\vspace{-20pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pics/alessio.jpg}}]{Dr. Alessio Del Bue}
(alessio.delbue@iit.it - Via Enrico Melen 83, 16152 Genova, Italy) is a tenured senior researcher at the PAVIS (Pattern Analyisis and computer VISion) Department of the Italian Institute of Technology (IIT) where he is leading the Visual Geometry and Modelling (VGM) Lab. His current research interests are related to 3D scene understanding from images and sound, 3D digitisation technology for Cultural Heritage studies, non-rigid image registration and reconstruction, and sensors/targets localisation and room reconstruction from sound.
\end{IEEEbiography}

\vspace{-20pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pics/fabio.jpg}}]{Dr. Fabio Galasso}
(f.galasso@osram.com - Parkring 33, 85748 Munich, Germany) heads the Computer Vision Department at OSRAM in Germany. The R\&D interests of the group involve computer vision, machine learning and multimodal computing, in relation to smart lighting applications. Specific activities regard detection, recognition, tracking and re-identification, the recognition and reconstruction of 3D scenes, domain adaptation and the estimation of lighting.
\end{IEEEbiography}

\vfill

==> sections/motivation.tex <==
\section{Motivation}

In this work we try to encompass both fundamental research in computer vision and innovation transfer in smart lighting,in order to push forward for a new generation of smart lighting systems for a better quality living and energy saving solutions. SMART Lighting is a novel field of research, whereby we try and bring together the new capabilities of lighting and the novel achievements of computer vision.

This study aims to create a breakthrough in light management systems by enabling the understanding of the environment via scene observation with cameras for smart illumination and energy saving. Thus, we applied research and developed novel autonomous tools using advanced computer vision and machine learning approaches that seamlessly can integrate into smart lighting systems for indoor environments. This can be applied with the use of a sensing device and implemented as a part of an artificial intelligence (AI) framework. The former could be a simple RGB camera (or RGBD if including a depth sensor, \eg ToF), co-located in a luminaire to provide top-views of the scene. The latter involves the algorithms to understand the scene and to make decisions on lighting, leading to the final idea of the \textit{“Invisible Light Switch”}.

Towards the understanding of the scene, we distinguish the scene structure material properties and the human-centric scene. The first regards the scene composition: meaning its 3D structure, the objects materials, the light position and characterization (natural versus artificial) and their lighting patterns. The second regards the human activities and interactions, particularly the human-scene (walking, working at desk or reading, presenting at a board) and human-human interaction (where people meet, discuss, relax, \etc).

Thereafter, the scene-centric composition analysis and human-centric scene understanding were combined towards a smart lighting management system with the key idea of \textit{"Invisible Light Switch"} (ILS), where the user have the sensation of \textit{"all lit"} while actually the scene is optimally lit, therefore providing both notable energy saving and a productive environment.

The idea behind the Invisible Light Switch is straightforward: the proposed system controls and sets the illumination of the environment by taking into account the information regarding the part of the scene that the user can see or cannot see, by switching off or dimming down the lights outside the user's View Frustum of Attention (VFOA), and thus ensuring a consistent energy saving and productivity. The study of the scene as discussed above serves this goal: knowing the 3D geometry of the scene and the map of interreflectances will allow to understand how the different light sources impact each point of the space; knowing where a user is located and what is his posture serves to infer what he can see and what he cannot, individuating potential areas where the light can be switched off. Moreover, being able to forecast his future activities will help understand (in advance) which lights should be switched on, avoiding the user to continuously act on the illumination system, and showing the user the illumination scenario that he wants to have.
